LIPEx-Locally Interpretable Probabilistic Explanations-To Look Beyond The True Class

In this work, we instantiate a novel perturbation-based multi-class explanation framework, LIPEx (Locally Interpretable Probabilistic Explanation). We demonstrate that LIPEx not only locally replicates the probability distributions output by the widely used complex classification models but also provides insight into how every feature deemed to be important affects the prediction probability for each of the possible classes. We achieve this by defining the explanation as a matrix obtained via regression with respect to the Hellinger distance in the space of probability distributions. Ablation tests on text and image data, show that LIPEx-guided removal of important features from the data causes more change in predictions for the underlying model than similar tests based on other saliency-based or feature importance-based Explainable AI (XAI) methods. It is also shown that compared to LIME, LIPEx is more data efficient in terms of using a lesser number of perturbations of the data to obtain a reliable explanation. This data-efficiency is seen to manifest as LIPEx being able to compute its explanation matrix around 53% faster than all-class LIME, for classification experiments with text data.

==> Notation.tex <==
\begin{document}


\section{Some Notation}\label{sec:note} 

\note{ 
 
The following come from the ``physics'' package except the inner-product~\\ ~\\
$\ip{\va}{\vb}, \abs{c}, \norm{\vd}, \pdv{L}{\vw}, \pdv[2]{L}{\vw}, \dv{W}{t}, \dd{x}, \rank (\mM),\tr(\mA),\Tr (\mB), \var{W}$
~\\ ~\\ 
$\relu$ is our definition
~\\ 
We have also defined the following calligraphic letters, 
$\cF, \cR, \cN, \cE, \cL, \cD$
~\\
}

\begin{center} 
\hl{This is the default highlight!}
\om{This is our customized highlight!}
\end{center} 

\note{ Everything below comes from the TMLR format \\
- which comes from this book, \url{https://github.com/goodfeli/dlbook_notation/}}

\vspace{0.5cm} 
\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\sA$ & A set\\
$\R$ & The set of real numbers \\
$\{0, 1\}$ & The set containing 0 and 1 \\
$\{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$[a, b]$ & The real interval including $a$ and $b$\\
$(a, b]$ & The real interval excluding $a$ but including $b$\\
$\sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\gG$ & A graph\\
$\parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\egroup 

~\\ ~\\
\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$a$ & A scalar (integer or real)\\
$\va$ & A vector\\
$\mA$ & A matrix\\
$\tA$ & A tensor\\
$\mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\mI$ & Identity matrix with dimensionality implied by context\\
$\ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\ra$ & A scalar random variable\\
$\rva$ & A vector-valued random variable\\
$\rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup

~\\ ~\\ 
\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup

~\\ ~\\ 
\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$P(\ra)$ & A probability distribution over a discrete variable\\
$p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup

~\\ ~\\ 
\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$ f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$ f \circ g $ & Composition of the functions $f$ and $g$ \\
$f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\log x$ & Natural logarithm of $x$ \\
$\sigma(x)$ & Logistic sigmoid, $\frac{1} {1 + \exp(-x)}$ \\
$\zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\norm{\vx}_p $ & $L^p$ norm of $\vx$ \\
$\norm{\vx}$ & $L^2$ norm of $\vx$ \\
$x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
$\argmax_{\rvx \in \R^n} f$\\  
$\argmin_{\rvx \in \R^n} f$\\
$\reg, \rect,\softmax,\sigmoid,\softplus,\Var,\standarderror$\\
\end{tabular}
\egroup

\end{document}


